Shaping Proto-Value Functions via Rewards

In this paper, we combine task-dependent reward shaping and task-independent proto-value functions to obtain reward dependent proto-value functions (RPVFs). In constructing the RPVFs we are making use of the immediate rewards which are available during the sampling phase but are not used in the PVF construction. We show via experiments that learning with an RPVF based representation is better than learning with just reward shaping or PVFs. In particular, when the state space is symmetrical and the rewards are asymmetrical, the RPVF capture the asymmetry better than the PVFs.

==> algo.tex <==
\section{Algorithm and Experiments}



==> raj.tex <==
Combinatorial laplacian operator is defined as $L=D-A $ where $D $ is the diagonal matrix whose entries are row sum of the adjacency matrix A. For any given function $ f:S \rightarrow \mathbb{R} $ which map the vertices of a graph (or state) to real number, the application of combinatorial Laplacian operator yields
\begin{align*}
Lf(u)=\Sigma_{v \sim u}(f(u)-f(v)) 
\end{align*}  
for every $v$ adjacent to $u$. The use of combinatorial Laplacian on a function $f$ on chain graph can be considered as the discrete counterpart of the famous Laplace partial differential equation.Consider ${v_i: i=1 \ldots N} $ are the vertices of a chain graph $G$ linked in to form a path of length $N$.
\begin{align*}
Lf(v_i) &=( f(v_i)-f(v_{i-1}) )+( f(v_i)-f(v_{i+1}) ) \\
       &=(f(v_i)-f(v_{i-1}) )-(f(v_{i+1})-f(v_i) ) \\
	&= \nabla (f(v_i,v_{i-1}))-\nabla (f(v_i,v_{i+1})) \\
	&=  \Delta (f(v_i))
\end{align*} 
Harmonic functions solves the equation $\Delta f=0 $. Eigen function of $\Delta $ are functios $f$ such that $\Delta f=\lambda f $ where $\lambda $ are the eigen value of $\Delta$.  When the domain is unit circle ; the trigonometric function $sin ,cos $ form the eigen function. So solving the Laplacian operator $L$ on a graph means finding the eigen value $\lambda $ and the eigen vector such that $Lf= \lambda f $ .
\par

A more sophisticated idea is normalized Laplacian which is similar to the non-symmetric random walk operator $D^{-1}A $. A diffusion model is intended to capture information flow on a graph or a manifold. A simple diffusion model is a random walk on an undirected graph, where the probability of transitioning from a vertex (state) to its neighbor is proportional to its degree, that is equals to the normalized Laplacian $P_r=D^{-1}A $. Simplicity is one of the key aqdvantages of the diffusion model and also it is easier to estimate than esimating the true transition matrix of the underlying graph of the MDP. This random walk operator is closely related (spectrally ) to the combinatorial Laplacian operator.

  

